The Challenges of Optimization For Data Science

Optimization problems arising in data science have given rise to a number of new derivative-based optimization methods. Such methods often use standard smoothness assumptions -- namely, global Lipschitz continuity of the gradient function -- to establish a convergence theory. Unfortunately, in this work, we show that common optimization problems from data science applications are not globally Lipschitz smooth, nor do they satisfy some more recently developed smoothness conditions in literature. Instead, we show that such optimization problems are better modeled as having locally Lipschitz continuous gradients. We then construct explicit examples satisfying this assumption on which existing classes of optimization methods are either unreliable or experience an explosion in evaluation complexity. In summary, we show that optimization problems arising in data science are particularly difficult to solve, and that there is a need for methods that can reliably and practically solve these problems.

==> section/notation.tex <==
\begin{table}[!ht]
    \centering
    \caption{Notation for Algorithm}
    \begin{tabular}{p{5cm} p{9cm}}
        \toprule
        $F(\theta), \dot{F}(\theta), \ddot{F}(\theta)$ & Objective, gradient of objective, and Hessian of objective, respectively.\\
        $k,j$ & Outer and inner loop iteration counters. \\
        $\theta_k$ & $k$th outer loop iterate. \\
        $\psi_j^k$ & $j$th inner loop iterate for outer loop iteration $k$.\\
        $\tau^k_{\iter,\exit}$ & Radius for bounding ball triggering event.\\
        $\tau^k_{\iter,\max}$ & Maximum inner loop iteration allowance.\\
        $\tau^k_{\gra,\upp}, \tau^k_{\gra,\low}$ & Upper and lower thresholds for gradient triggering event.\\
        $\delta, \delta_k$ & Step size scaling term.\\
        $\tau^k_{\obj}$ & Nonmonotone search threshold.\\
        $w$ & Number of objective values in nonmonotone search.\\
        $\rho$ & Relaxation term in nonmonotone Armijo condition.\\
        $\sigma_{\upp}, \sigma_{\low}$ & Inflation and Reduction factors for step size scaling term.\\
        $\alpha, \alpha_j^k, \mathrm{StepSize}$ & Step size, and the function that produces the step size.\\
        $\gamma, \gamma_j^k, \mathrm{StepDirection}$ & Step applied to each inner loop iterate, and the function that produces the step.\\
        $\epsilon$ & Gradient threshold for termination.\\
        $\hat{L}_j^k$ & Approximation of local Lipschitz constant\\\bottomrule
    \end{tabular}
\end{table}

\begin{table}[!ht]
    \centering
    \caption{Notation for Theory}
    \begin{tabular}{p{5cm} p{9cm}}
        \toprule
        $\mathbb{N}, \mathbb{R}^n$ & Natural numbers, n-dimensional Euclidean space.\\
        $\inlinenorm{\cdot}_2$ & Euclidean norm. \\
        $C, C_k, C_u'$ & Compact sets. \\
        $\underline g(C)$ & Constant in compact set $C$ to ensure step direction is a descent direction. See \cref{property-stepdirection-negative}. \\
        $\overline g(C)$ & Constant in compact set $C$ to ensure the norm of step direction is within some factor of the norm gradient. See \cref{property-stepdirection-propgrad}. \\
        $\overline \alpha(C)$ & Upper bound on step size in compact set $C$. See \cref{property-stepsize-upper}. \\
        $\underline \alpha(C)$ & Lower bound on step size in compact set $C$. See \cref{property-stepsize-lower}.\\
        $\overline \tau_{\exit}(\theta)$ & Upper bound on radius for bounding ball. See \cref{property-radius-bounded}.\\
        $\overline \tau_{\max}$ & Upper bound on maximum number of inner loop iterations. See \cref{property-iter-max}.\\
        $\mathcal{B}(\theta), \mathcal{B}(\theta, R)$ & Ball around $\theta$. Radius either specified implicitly or with $R$.\\
        $\mathcal{G}(\theta), \mathcal{G}(\theta, R)$ & Max norm gradient within the ball $\mathcal{B}(\theta)$ or $\mathcal{B}(\theta, R)$.\\
        $\mathcal{L}(C)$ & Local Lipschitz constant within compact set $C$.\\
        $\ell_k$ & Index of iterates that satisfied the nonmonotone Armijo Condition.\\
        $L(k)$ & Sub-index of last accepted iterate.\\
        $O(k)$ & Largest sub-index smaller than $L(k)$ such that $\ell_{O(k)}$ is the index of the iterate, whose objective value is used as the nonmonotone threshold.\\
        $o_s$ & Sub-index such that $\ell_{o_s}$ are the indices of the iterates, whose objective values are used as nonmonotone thresholds.\\
        $g_u$ & Subindices for $\ell$ of distinct iterates used in analysis of the gradient.\\\bottomrule
    \end{tabular}
\end{table}

==> section/smoothness-of-ds-problems/poisson-reg/poisson-reg.tex <==
Poisson regression is a common tool for modeling the behavior of count data as a function of regressors. As a trivial example developed in \cite[Section B.4]{patel2021globalconvergence}, we consider regressing a Poisson variable, $Y$, on an independent Poisson variable, $Z$, both with mean $1$. As the variables are independent, the true parameter is zero. However, if we still try to perform the regression, then the expected negative log-likelihood is $F(\theta) = - \theta + \exp(\exp(\theta) - 1)$, which is minimized at $\theta = 0$ \cite[see][Section B.4]{patel2021globalconvergence}. 

The gradient and Hessian are
\begin{equation}
\dot F(\theta) = -1 + \exp(\exp(\theta) + \theta -1 ),\quad\text{and}\quad \ddot F(\theta) = (\exp(\theta) + 1)\exp( \exp(\theta) + \theta - 1),~\text{respectively}.
\end{equation}

We now check the aforementioned smoothness conditions.
\begin{remunerate}
\item As $\ddot F(\theta)$ tends to $\infty$ as $\theta \to \infty$, $F$ is \textbf{not} globally Lipschitz smooth.
\item Note, $\ddot F(0) = 2$. Now,
\begin{equation}
\lim_{\theta \to \infty} \frac{|\ddot F(\theta) - \ddot F(0)|}{|\theta - 0|} \geq \lim_{ \theta \to \infty} \frac{\exp(\theta) + 1}{|\theta|} = \infty.
\end{equation}
Hence, $F$ is \textbf{not} globally Lipschitz Hessian smooth.
\item Now, $|\dot F(\theta)|$ tends to $\infty$ only when $\theta$ goes to $\infty$. Then,
\begin{align}
\limsup_{\theta \to \infty } \frac{\dot F (\theta)^2 }{|\ddot F(\theta)| } 
&= \limsup_{\theta \to \infty} \frac{\exp(2 \exp(\theta) + 2\theta - 2) - 2\exp( \exp(\theta) + \theta - 1) + 1}{\exp( \exp(\theta) + 2 \theta - 1) + \exp(\exp(\theta) + \theta - 1)} \\
&\geq \limsup_{\theta \to \infty} \frac{\exp(2 \exp(\theta) + 2\theta - 2) - 2\exp( \exp(\theta) + \theta - 1)}{\exp( \exp(\theta) + 2 \theta - 1)} \\
&\geq \limsup_{\theta \to \infty} \exp( \exp(\theta) - 1) - 2 \exp(-\theta).
\end{align}
The right hand side of the last inequality is infinity. Accordingly, $F$ is \textbf{not} subquadratically Lipschitz smooth; $F$ is \textbf{not} quadratically Lipschitz smooth. $F$ is superquadratically Lipschitz smooth.
\end{remunerate}

==> section/smoothness-of-ds-problems/poisson-reg/smoothness-proof.tex <==
For $\theta > 0$, note that $\exp\bigpar{\theta x}$ is a convex function. Therefore, for $\theta > 0$ and letting $\bar{x}$ denote the sample average of data points $x_i$, we can apply Jensen's inequality (as $x_i > 0$) to obtain
\begin{equation}
    \begin{aligned}
        \abs{\dot{\ell}(\theta) - \dot{\ell}(0)} &= \abs{\sum_{i=1}^n \exp\bigpar{\theta x_i} x_i - x_i } \ge \sum_{i=1}^n \exp\bigpar{\theta x_i} x_i - n\bar{x} = n\bar{x}\sum_{i=1}^n \exp\bigpar{\theta x_i} \frac{x_i}{n\bar{x}} - n\bar{x}\\ 
        &\ge n\bar{x}\exp\bigpar{\theta \sum_{i=1}^n \frac{x_i^2}{n\bar{x}}} - n\bar{x}
    \end{aligned}
\end{equation}
Since $\exp\bigpar{\theta \sum_{i=1}^n \frac{x_i^2}{n\bar{x}}} \to \infty$ as $\theta \to \infty$ we have for any $L > 0$, that there exists a $\theta_*$ such that 
\begin{equation}
    L \le \frac{\abs{n\bar{x}\exp\bigpar{\theta_*\sum_{i=1}^n \frac{x_i^2}{n\bar{x}}} - n\bar{x}}}{\abs{\theta_*}} \le \frac{\abs{\dot{\ell}(\theta_*) - \dot{\ell}(0)}}{\abs{\theta_*}}
\end{equation}
Which implies that the gradient cannot be globally Lipschitz continuous. We apply essentially the same proof for the Hessian, namely for $\theta > 0$ and letting $\overline{x^2} = n^{-1}\sum_{i=1}^n x_i^2$
\begin{equation}
    \begin{aligned}
        \abs{\ddot{\ell}(\theta) - \ddot{\ell}(0)} &= \abs{\sum_{i=1}^n x_i^2 \bigpar{\exp\bigpar{\theta x_i} - 1}} \ge n\overline{x^2} \sum_{i=1}^n \exp\bigpar{\theta x_i} \frac{x_i^2}{n\overline{x^2}} - n\overline{x^2}\\
        &\ge n\overline{x^2}\exp\bigpar{\theta \sum_{i=1}^n \frac{x_i^3}{n\overline{x^2}}} - n\overline{x^2}
    \end{aligned}
\end{equation}
By the same argument as in the gradient case, we get that the hessian is not globally Lipschitz continuous. Finally, to show that $\inlinenorm{\ddot{\ell}(\theta)}$ is not bounded above by a sub-quadratic function of $\inlinenorm{\dot{\ell}(\theta)}$, we show when $\{(x_i, y_i)\}_{i=1}^n = \{(-1,0)\}$ that
\todo{This isn't right...}
